Efficient Algorithms for Personalized PageRank

We present new, more efficient algorithms for estimating random walk scores such as Personalized PageRank from a given source node to one or several target nodes. These scores are useful for personalized search and recommendations on networks including social networks, user-item networks, and the web. Past work has proposed using Monte Carlo or using linear algebra to estimate scores from a single source to every target, making them inefficient for a single pair. Our contribution is a new bidirectional algorithm which combines linear algebra and Monte Carlo to achieve significant speed improvements. On a diverse set of six graphs, our algorithm is 70x faster than past state-of-the-art algorithms. We also present theoretical analysis: while past algorithms require $\Omega(n)$ time to estimate a random walk score of typical size $\frac{1}{n}$ on an $n$-node graph to a given constant accuracy, our algorithm requires only $O(\sqrt{m})$ expected time for an average target, where $m$ is the number of edges, and is provably accurate. In addition to our core bidirectional estimator for personalized PageRank, we present an alternative algorithm for undirected graphs, a generalization to arbitrary walk lengths and Markov Chains, an algorithm for personalized search ranking, and an algorithm for sampling random paths from a given source to a given set of targets. We expect our bidirectional methods can be extended in other ways and will be useful subroutines in other graph analysis problems.

==> scratch_writing.tex <==
\section{(Old) Itemized contributions}

This thesis contains the following contributions:
\begin{enumerate}
\item A bidirectional estimator \bippr{} which is at least 70x faster than previous algorithms at estimating Personalized PageRank scores to within 10\% relative error on a diverse set of six graphs, ranging in size from millions to billions of edges.  See Section \ref{sec:bippr_experimental_time}.
\item \bippr{} can estimate a Personalized PageRank score of size greater than $1/n$ within relative error $\epsilon$ with probability $1 - \pfail$ in expected time 
\[O \pn{ \frac{\log \frac{1}{\pfail}}{\epsilon} \sqrt{m} }\]
 for a uniform random target on a worst-case graph.  This estimator also applies to standard (global) PageRank, giving the best known running time for estimating the global PageRank of a single node.  See Section \ref{sec:bippr}, Theorem \ref{thm:fastpprtime}.  
  \item \bippr{}, given pre-computation time and space of  $ O \pn{n \frac{\log \frac{1}{\pfail}}{\epsilon} \sqrt{m} }$,  can achieve the same guarantee in worst-case time 
\[O \pn{\sqrt{m} \frac{\log \frac{1}{\pfail}}{\epsilon}}.\]
See Section \ref{sec:bippr}, Theorem (todo) \ref{thm:fastpprtime}.
  \item \bippr{} can estimate a score $\pi_s[t]$ with the same guarantees using worst-case time 
\[O \pn{ \frac{\log \frac{1}{\pi_s[t]}}{\epsilon} \sqrt{\frac{d^*}{\pi_s[t]}}}\]
 where $d^*$ is the average in-degree of a certain set of nodes (see section todo for details).  See Section \ref{sec:bippr}, Theorem (todo).

  \item An alternative bidirectional estimator for undirected graphs. On such graphs, the natural global importance of a node $t$ is $d_t / m$, since this is the probability of stopping at $t$ as the walk length goes to infinity, so only Personalized PageRank scores larger than $d_t / m$ are interesting.  This estimator can  estimate a Personalized PageRank score $\pi_s[t]$ of size greater than $d_t/m$  within relative error $\epsilon$ with probability $1 - \pfail$ in expected time 
\[O \pn{ \frac{\log \frac{1}{\pfail}}{\epsilon} \sqrt{m}}\]
 for a worst-case target $t$ and worst-case undirected graph.  See Section \ref{sec:ubippr}, Theorem \ref{thm:worstcase}.

\item A generalized bidirectional estimator that can estimate $\ell$-step transition probabilities on any weighted graph (or Markov Chain) from any source distribution to any target within relative error $\epsilon$ with probability $1 - \pfail$. For a uniform random target, if the estimated probability is greater than $\delta$, the expected running time is 
\[O \pn{\frac{\log \frac{1}{\pfail}}{\epsilon} \ell^{3/2}\sqrt{\dbar/\delta}}. \]
See Chapter \ref{sec:mc_chapter}.
\item A personalized search algorithm which can efficient respond to name search queries. In experiments on a 1.5 billion edge Twitter graph, this algorithm is more efficient than past algorithms (see todo).  Given $O(n \sqrt{m})$ precomputation time and space, this algorithm can respond to name search queries with provable approximate accuracy guarantees in time $O(\sqrt{m})$.  See todo.
\item An algorithm which given start $s$ and target $t$ (or a set of targets) can sample a random path from $s$ conditioned on stopping at $t$.  Its average expected running time is
\[O \pn{\sqrt{m}}\]
for a uniform random target.
\end{enumerate}


==> tmp_bippr.tex <==
\section{Bidirectional-PPR}
\label{sec:bippr}
In this section we present our new bidirectional algorithm for PageRank estimation \cite{bippr}. %We describe the algorithm, given an example, prove accuracy and efficiency guarantees, and finally describe a practical running time improvement.
At a high level, our algorithm estimates $\pi_s[t]$ by first working backwards from $t$ to find a set of intermediate nodes `near' $t$ and then generating random walks forwards from $s$ to detect this set.  Our method of combining reverse estimates with forward random walks is based on the residual vector returned by the \rpush{} algorithm (given in Section \ref{sec:reverse_push} as Algorithm \ref{alg:invPPR}) of Andersen et.~al.~\cite{Andersen2007}.  Our \bippr{} algorithm is based on the observation that in order to estimate $\pi_s[t]$ for a \emph{particular} $(s, t)$ pair, we can boost the accuracy of \rpush{} by sampling random walks from $s$ and incorporating the residual values at their endpoints.

\subsection{The \bippr{} Algorithm}
The reverse work from $t$ is done via the \rpush{}$(t, \rmax, \alpha)$, where $\rmax$ is a parameter we discuss more in Section \ref{sec:balancing}.  Recall from Section \ref{sec:reverse_push} that this algorithm produces two non-negative vectors $p^t \in \R^n$ (estimates) and $r^t \in \R^n$ (residual messages) which satisfy the following invariant (Lemma $1$ in \cite{Andersen2007})
\begin{equation}
  \label{eq:ppr_dot_product}
  \pi_s[t] = p^t[s] + \sum_{v \in V} \pi_s[v] r^t[v].
\end{equation}
The central idea is to reinterpret Equation \eqref{eq:ppr_dot_product} as an expectation:
\begin{equation}
  \label{eq:ppr_expectation}
  \pi_s[t] = p^t[s] + \EE_{v \sim \pi_s}[r^t[v]]. \end{equation}
Now, since $\max_v r^t[v] \leq \epr$, the expectation $\EE_{v \sim \pi_s[v]}[r^t[v]]$ can be efficiently estimated using Monte Carlo.  
To do so, we generate $w = c \frac{\epr}{\delta}$ random walks of length $Geometric(\alpha)$ from start node $s$. This choice of $w$ is  based on Theorem \ref{thm:bidirmain}, which provides a value for $c$ based on the desired accuracy, and here $\delta$ is the minimum PPR value we want to accurately estimate.  
Let $V_i$ be the final node of the $i$th random walk. From Equation \ref{eq:defmc}, $\Pr[V_i=v] = \pi_s[v]$.  Our algorithm returns the natural emperical estimate for Equation \ref{eq:ppr_expectation}:
%Let $X_i = r^t[V_i]$ denote the residual from the final node of the $i$th random walk, and $\bar{X} = \frac{1}{w} \sum_{i=1}^w X_i$. 
%Then \bippr{} returns as an estimate of $\pi_s[t]$: 
\[\widehat{\pi}_s[t] = p^t[s] + \frac{1}{w}\sum_{i=1}^w r^t[V_i]
\]
The complete pseudocode is given in Algorithm \ref{alg:BIPPR}.


\begin{algorithm}[!ht]
\caption{\bippr{}$(s,t,\delta)$}
\label{alg:BIPPR}
\begin{algorithmic}[1] 
\REQUIRE graph $G$, teleport probability $\alpha$, start node $s$, target node $t$, minimum probability $\delta$, accuracy parameter $c$ (in our experiments we use $c = 7$)

\STATE $(p_t, r_t)$ =  \rpush{}$(t,\epr, \alpha)$

\STATE Set number of walks $w=c \epr/\delta$ \quad(cf. Theorem \ref{thm:bidirmain})
\FOR{index $i\in [w]$}
\STATE Sample a random walk starting from $s$ (sampling a start from $s$ if $s$ is a distribution), stopping after each step with probability $\alpha$, and let $V_i$ be the endpoint
%\STATE Set $X_i = r_t[V_i]$
\ENDFOR 
\RETURN $\widehat{\PR}_s[t]=p_t[s] + (1/w)\sum_{i\in[w]} r_t[V_i]$
\end{algorithmic}
\end{algorithm}

As an example, consider the graph in Figure \ref{fig:example_9node_graph}.
\begin{figure}[tbph]
  \centering
  \includegraphics[width=0.9\columnwidth]{example_9node_graph}
  \caption{An example graph.  We will estimate $\pi_s[t]$.}
  \label{fig:example_9node_graph}
\end{figure}
Suppose we run \rpush{} on this graph with target $t$ and teleport probability $\alpha$ to accuracy $\rmax=0.11$.  The resulting PPR estimates $p$ and residuals $r$ are shown in Figure \ref{fig:example_9node_iteration5}.
\begin{figure}[tbph]
  \centering
  \includegraphics[width=0.9\columnwidth]{example_9node_iteration5}
  \caption{An example graph.  We will estimate $\pi_s[t]$.}
  \label{fig:example_9node_iteration5}
\end{figure}
In the second phase of the algorithm we take random walks forwards. If we set minimum PPR $\delta=0.01$ and chernoff constant, $c=7$, the number of walks we need to do is 
$ w = c \frac{\rmax}{\delta} = 77$
If we perform 77 walks, we might get the empirical forward probabilities $\tilde{\pi}_s$ shown in Figure \ref{fig:example_9node_pp}.
\begin{figure}[tbph]
  \centering
  \includegraphics[width=0.9\columnwidth]{example_9node_pp}
  \caption{The empirical probability of stopping at each node after 77 walks from $s$ for some choice of random seed.  Note there is an implicit self loop at $v$.}
  \label{fig:example_9node_pp}
\end{figure}
If we look at the residuals $r$ from Figure \ref{fig:example_9node_iteration5} and the forward probabilities $\tilde{\pi}_s$ in Figure \ref{fig:example_9node_pp} we see the only node with nonzero value on both happens to be $c$, so our estimate for this run of the algorithm is
\[\hat{\pi}_s[t] = p^t[s] + \sum_v \tilde{\pi}_s[v] r^t[v] = 0 + 0.13 \cdot 0.1 = 0.013. \]

%\subsection{Analysis}
\subsection{Accuracy Analysis}
We first prove that  high probability, \bippr{} returns an estimate with small relative error if $\pi_s[t]$ is above a given threshold, and returns an estimate with small additive error otherwise.
\begin{theorem}
\label{thm:bidirmain} 
Given start node $s$ (or source distribution $\sigma$), target $t$, minimum PPR $\delta$, maximum residual $\epr > \frac{2e \delta}{\alpha \epsilon}$, relative error $\epsilon \leq 1$, and failure probability $\pfail$, \bippr{} outputs an estimate $\widehat{\PR}_s[t]$ such
that with probability at least $1- \pfail$ the following hold: 
\begin{itemize}[nosep,leftmargin=*]
\item If $\pi_s[t] \geq \delta$: \hspace{1cm} $\abs{\pi_s[t]-\hat{\pi}_s[t]} \leq \epsilon \pi_s[t]$. 
\item If $\pi_s[t] \leq \delta$: \hspace{1cm}
%$\abs{\pi_s[t]-\hat{\pi}_s[t]} \leq \frac{\epsilon^2}{3 \ln(2)} \delta$.
$\abs{\pi_s[t]-\hat{\pi}_s[t]} \leq 2e\delta$.
\end{itemize}
\end{theorem}
The above result shows that the estimate $\hat{\pi}_s[t]$ can be used to distinguish between `significant' and `insignificant' PPR pairs: for pair $(s,t)$, Theorem \ref{thm:bidirmain} guarantees that if $\pi_s[t] \geq \frac{(1+2e)\delta}{(1-\epsilon)}$, then the estimate is greater than $(1+2e)\delta$, whereas if $\pi_s[t] < \delta$, then the estimate is less than $(1+2e)\delta$. 
The assumption $\epr > \frac{2e \delta}{\alpha \epsilon}$ is easily satisfied, as typically $\delta=O\pn{\frac{1}{n}}$ and $\rmax =\Omega\pn{\frac{1}{\sqrt{m}}}$.

\begin{proof} 
%(Based on the proof in \cite{generalized_fastppr}).
As shown in Algorithm \ref{alg:BIPPR}, we will average over 
\[ w = c \frac{\epr}{\delta}, \]
walks, where $c$ is a parameter we choose later.
Each walk is of length $Geometric(\alpha)$, and we denote $V_i$ as the last node visited by the $i^{th}$ walk so that $V_i\sim\pi_s$.
Now let $X_i = r^t[V_i]$.  The estimate returned by \bippr{} is:
\[\widehat{\pi}_s[t] = p^t[s] + \frac{1}{w} \sum_{i=1}^w X_i. \]
First, from Equation \eqref{eq:ppr_dot_product}, we have that $\EE[\widehat{\pi}_s[t]]= \pi_s[t]$, that is, our estimate is unbiased.   
Since \rpush{} guarantees that for all $v$, $r^t[v]<\epr$, each $X_i$ is bounded in $[0,\epr]$.  Before we apply Chernoff bounds, we rescale $X_i$ by defining $Y_i = \frac{1}{\epr} X_i \in [0,1]$. We also define $Y = \sum_{i=1}^w Y_i$

We show concentration of the estimate via the following two Chernoff bounds (see Theorem $1.1$ in~\cite{DuPa09}):
\begin{enumerate}
\item $\PP[|Y - \EE[Y]| > \epsilon \EE[Y]] < 2 \exp(-\frac{\epsilon^2}{3}\EE[Y])$
\item $\textrm{For any } b > 2e\EE[Y], \PP[Y > b] \leq 2^{-b}$
\end{enumerate}
We perform a case analysis based on whether $\EE[X_i] \geq \delta$ or $\EE[X_i] < \delta$. 

First suppose $\EE[X_i] \geq \delta$.  Note that this implies that $\pi_s[t] \geq \delta$ so we will prove a relative error bound of $\epsilon$.
Now we have $\EE[Y] = \frac{w}{\epr} \EE[X_i] = \frac{c}{\delta} \EE[X_i] \geq c$, and thus:
\begin{align*}
\PP[\abs{\widehat{\pi}_s[t] - \pi_s[t]} > \epsilon \pi_s[t]] 
 &\leq \PP[\abs{\bar{X} - \EE[X_i]} > \epsilon \EE[X_i]] \\
  &= \PP[\abs{Y - \EE[Y]} > \epsilon \EE[Y]] \\
  &\leq 2 \exp\pn{-\frac{\epsilon^2}{3}\EE[Y]} \\
  &\leq 2 \exp\pn{-\frac{\epsilon^2}{3} c}
  \leq \pfail,
\end{align*}
where the last line holds as long as we choose
\[ c \geq \frac{3}{\epsilon^2} \ln \pn{\frac{2}{\pfail}}.\]
%This case is concluded because if $\abs{\bar{X} - \EE[X_i]} \leq \epsilon \EE[X_i]$ then $\abs{\widehat{\pi_s[t]} - \pi_s^t} \leq \epsilon \pi_s^t$.

Suppose alternatively that $\EE[X_i] < \delta$.  Then
\begin{align*}
\PP[\abs{\hat{\pi}_s[t] - \pi_s[t]} > 2e\delta]
&= \PP[\abs{\bar{X} - \EE[X_i]} > 2e\delta] \\
%&=  \PP\bk{\abs{\frac{\epr}{w} Y - \frac{\epr}{w} \EE[Y]} > 2e\delta} \\
&=  \PP\bk{\abs{Y -  \EE[Y]} > \frac{w}{\epr} 2e\delta} \\
&\leq  \PP\bk{Y > \frac{w}{\epr}2e\delta} .
\end{align*}
At this point we set $b = \frac{w}{\epr} 2e\delta=2ec$ and apply the second Hoeffding bound.  Note that $\EE[Y] = \frac{c}{\delta} \EE[X_i] < c$, and hence we satisfy $b > 2e \EE[Y]$.
The second bound implies that
\begin{equation}
  \label{eq:1}
   \PP[\abs{\hat{\pi}_s[t] - \pi_s[t]} > 2e\delta] \leq 2^{-b} \leq \pfail
\end{equation}
as long as we choose $c$ such that:
\[ c \geq \frac{1}{2e} \log_2 \frac{1}{\pfail}. \]
If  $\pi_s[t] \leq \delta$, then equation \ref{eq:1} completes our proof. 

% where the last line holds if we choose
% \[ c = \frac{3}{\epsilon^2} \ln \pn{\frac{2}{\pfail}}.\]
% %This case is concluded because if $\abs{\bar{X} - \EE[X_i]} \leq \epsilon \EE[X_i]$ then $\abs{\widehat{\pi_s[t]} - \pi_s^t} \leq \epsilon \pi_s^t$.

% Suppose alternatively that $\EE[X_i] < \delta$.  Then
% \begin{align*}
% \PP[\abs{\hat{\pi}_s[t] - \pi_s[t]} > \frac{\epsilon^2}{3 \ln(2)} \delta]
% &= \PP[\abs{\bar{X} - \EE[X_i]} > \frac{\epsilon^2}{3 \ln(2)} \delta] \\
% %&=  \PP\bk{\abs{\frac{\epr}{w} Y - \frac{\epr}{w} \EE[Y]} > 2e\delta} \\
% &=  \PP\bk{\abs{Y -  \EE[Y]} > \frac{w}{\rmax}\frac{\epsilon^2}{3 \ln(2)} \delta} \\
% &\leq  \PP\bk{Y > \frac{w}{\rmax}\frac{\epsilon^2}{3 \ln(2)} \delta } .
% \end{align*}
% At this point we set $b = \frac{w}{\rmax}\frac{\epsilon^2}{3 \ln(2)} \delta = \frac{c \epsilon^2}{3 \ln(2)} = \frac{\ln \pn{\frac{2}{\pfail}}}{\ln(2)} \geq -\log_2(\pfail)$ and apply the second Hoeffding bound.  Note that (todo) $\EE[Y] = \frac{c}{\delta} \EE[X_i] < c$, and hence we satisfy $b > 2e \EE[Y]$.
% The second bound implies that
% \begin{equation}
%   \label{eq:1}
%    \PP[\abs{\hat{\pi}_s[t] - \pi_s[t]} > \frac{\epsilon^2}{3 \ln(2)} \delta ] \leq 2^{-b} \leq \pfail
% \end{equation}
% as long as we choose $c$ such that:
% \[ c \geq \frac{1}{2e} \log_2 \frac{1}{\pfail}. \]
%If  $\pi_s[t] \leq \delta$, then equation \ref{eq:1} completes our proof. 

The only remaining case is when $\pi_s[t] > \delta$ but $\EE[X_i] < \delta$. This implies that $p^t[s] > 0$ since $\pi_s[t] = p^t[s] + \EE[X_i]$.  In the \rpush{} algorithm when we increase $p^t[s]$, we always increase it by at least $\alpha \rmax$, so we have $\pi_s[t] \geq \alpha \rmax$.  We have that
\[ \frac{\abs{\hat{\pi}_s[t] - \pi_s[t]}}{\pi_s[t]} \leq \frac{\abs{\hat{\pi}_s[t] - \pi_s[t]}}{\alpha \rmax}. \]
By assumption, $\frac{2e \delta}{\alpha \rmax} < \epsilon$, so by equation \ref{eq:1},
\[ \PP\bk{\frac{\abs{\hat{\pi}_s[t] - \pi_s[t]}}{\pi_s[t]} > \epsilon} \leq \pfail \]

The proof is completed by combining all cases and choosing $c = \frac{3}{\epsilon^2} \ln \pn{\frac{2}{\pfail}}$.  
We note that the constants are not optimized; in experiments we find that $c=7$ gives mean relative error less than 8\% on a variety of graphs.
\end{proof}

\subsection{Running Time Analysis}
\label{sec:bippr_running_time}

The runtime of \bippr{} depends on the target $t$: if $t$ has many in-neighbors and/or large global PageRank $\pi[t]$, then the running time will be slower because the reverse pushes will iterate over a large number of nodes.  For example, in the worst case, we might have $\indegree{t} = \Theta(n)$ and \bippr{} takes $\Theta(n)$ time.  However, we can give an average case analysis, and in Section \ref{sec:parameterized_bippr} we give a back-of-the-envelope  parameterized running time estimate.

\subsubsection{Average Case Running Time Analysis}
Alternatively, for \emph{a uniformly chosen target node}, we can prove the following:
\begin{theorem}
\label{thm:fastpprtime} 
For any start node $s$ (or source distribution $\sigma$), minimum PPR $\delta$, maximum residual $\epr$, relative error $\epsilon$, and failure probability $\pfail$, if the target $t$ is chosen uniformly at random, then \emph{\bippr{}} has expected running time
\[ O\pn{ \sqrt{\frac{\bar{d}}{\delta}} \frac{\sqrt{\log\pn{1/\pfail}}}{\alpha \epsilon}}.
 \]
\end{theorem}

In contrast, the running time for \texttt{Monte-Carlo} to achieve the same accuracy guarantee is $O\pn{\frac{1}{\delta} \frac{\log\pn{1/\pfail}}{\alpha \epsilon^2}}$, and the running time for \rpush{} is $O\pn{\frac{\bar{d}}{\delta \alpha}}$.  The \texttt{FAST-PPR} algorithm of \cite{fastppr} has an average running time bound of
$O\pn{\frac{1}{\alpha\epsilon^2}\sqrt{\frac{\bar{d}}{\delta}} \sqrt{ \frac{\log\pn{1/\pfail} \log\pn{1/\delta}}{\log\pn{1/(1-\alpha)}} }}$
 for uniformly chosen targets.  
The running time bound of \bippr{} is thus asymptotically better than \texttt{FAST-PPR}, and in our experiments (Section \ref{sec:bippr_experimental_time}) \bippr{} is significantly faster than past algorithms. %In experiments we find that \bippr{} is 3 to 8 times faster on a diverse set of graphs.
% Typical values might be $\pfail = 10^{-6}$, $\epsilon = \frac{1}{10}$ (since PPR values vary over a large range, even a constant relative error provides allows them to be ranked accurately), and $\delta = \frac{1}{n}$ (this is the average value of $\pi_s$, so if $\pi_s[t] < \frac{1}{n}$ then $t$ is not very relevant to $s$).  

\begin{proof} 
We first show that for a uniform random $t$, \rpush{} runs in average time $\frac{\bar{d}}{\alpha \epr}$ where $\bar{d}$ is the average degree of a node. This is because each time we push from a node $v$, we increase $p^t[v]$ by at least $\alpha \rmax$.  Since $p^t[v] \leq \pi_v[t]$ and $\sum_t \pi_v[t] = 1$, this lets us bound the average running time:
\begin{align*}
 &\frac{1}{n} \sum_{t \in V} \sum_{v \in V} \indegree{v}  [\text{\# times $v$ is pushed during \rpush{}($t, \rmax, \alpha$)}] \\
 &\leq \frac{1}{n} \sum_{t \in V} \sum_{v \in V} \indegree{v} \frac{\pi_v[t]}{\alpha \rmax} \\
 &\leq \frac{1}{n} \sum_{v \in V} \indegree{v} \frac{1}{\alpha \rmax} \\
& \leq \frac{\dbar}{\alpha \rmax}.
\end{align*}
  On the other hand, from Theorem \ref{thm:bidirmain}, the number of walks generated is
$O\pn{ \frac{\epr}{\delta\epsilon^2} \ln\pn{1/\pfail}}$ random walks, each of which can be sampled in average time $1/\alpha$.  Finally, we choose $\epr = \epsilon \sqrt{\frac{\bar{d} \delta}{ \ln\pn{2/\pfail}}}$ to minimize our running time bound and get the claimed result. 
\end{proof}

\subsubsection{A Practical Improvement: Balancing Forward and Reverse Running Time}
\label{sec:balancing}

The dynamic runtime-balancing heuristic proposed in \cite{fastppr} can improve the running time of Bidirectional-PageRank in practice.  In this technique, $\epr$ is chosen dynamically in order to balance the amount of time spent by \rpush{} and the amount of time spent generating random walks. 
To implement this, we modify \rpush{}  to use a priority queue in order to always push from the node $v$ with the largest value of $r_t[v]$.  
Then we change the the while loop so that it terminates when the amount of time spent achieving the current value of $\epr$ first exceeds the predicted amount of time required for sampling random walks, $c_{\text{walk}}  \cdot c \cdot \frac{\epr}{\delta}$, where $c_{\text{walk}}$ is the average time it takes to sample a random walk.  For a plot showing how using a fixed value for $\rmax$ results in unbalanced running time for many targets, and how this variant empirically balances the reverse and forward times, see \cite{fastppr}.  
The complete pseudocode is given as Algorithm \ref{alg:invPPRBalanced} 
\begin{algorithm}[!ht]
\caption{\texttt{\rpush{}Balanced}$(G, t, \alpha, \delta)$~\cite{Andersen2007}}
\label{alg:invPPRBalanced}
\begin{algorithmic}[1]
\REQUIRE graph $G$ with edge weights $w_{u,v}$, teleport probability $\alpha$, target node $t$, minimum probability $\delta$, accuracy parameter $c$ (in our experiments we use $c = 7$)
\STATE Choose tuning constant $c_{\text{walk time}}$, the average time it takes to generate a walk.
\STATE Initialize (sparse) estimate-vector $p^t = \vec{0}$ and (sparse) residual-vector $r^t = e^t$ (i.e.~$r^t(v) = 1$ if $v=t$; else $0$)
\STATE Initial Max-Priority-Queue $q$ with priority $r^t$
\STATE Start stopwatch $w$
\STATE Define function forwardTime($\rmax$) = $ c_{\text{walk time}} c \frac{\rmax}{\delta}$
\WHILE{$Q$.nonEmpty() and $w\text{.elapsedTime()} < \text{forwardTime($Q$.maxPrioriority())}$}
\STATE Let $v = Q.\text{popMax()}$
\FOR{$u\in \inneighbors{v}$}
   \STATE $r^t(u) \pluseq (1 - \alpha) w_{u,v} r^t(v)$ (increasing $u$'s priority in $Q$)
\ENDFOR
\STATE      $p^t(v) \pluseq \alpha r^t(v)$
\STATE      $r^t(v)=0$ 
\ENDWHILE
\STATE $\rmax = Q$.maxPriority() if $Q$ is non-empty, otherwise $\rmax=0$
\RETURN $(p^t, r^t, \rmax)$
\end{algorithmic}
\end{algorithm}    
and Algorithm \ref{alg:BIPPR_balanced}.
\begin{algorithm}[!ht]
\caption{\texttt{Bidirectional-PPR-Balanced}$(s,t,\delta)$}
\label{alg:BIPPR_balanced}
\begin{algorithmic}[1] 
\REQUIRE graph $G$, teleport probability $\alpha$, start node $s$, target node $t$, minimum probability $\delta$, accuracy parameter $c$ (in our experiments we use $c = 7$)

\STATE $(p^t, r^t, \rmax)$ =  \texttt{ReversePushBalanced}$(G, t, \alpha, \delta)$

\STATE Set number of walks $w=c \epr/\delta$ \quad(for $c$'s value, see Theorem \ref{thm:bidirmain}; we use $c=7$ in experiments)
\FOR{index $i\in [w]$}
\STATE Sample a random walk starting from $s$ (sampling a start from $s$ if $s$ is a distribution), stopping after each step with probability $\alpha$; let $V_i$ be the endpoint
\STATE Set $X_i = r^t[V_i]$
\ENDFOR 
\RETURN $\widehat{\PR}_s[t]=p^t[s] + (1/w)\sum_{i\in[w]}X_i$
\end{algorithmic}
\end{algorithm}


\subsubsection{Choosing the Minimum Probability  $\delta$}
\label{sec:choosing_delta} 
%\inlineheading{Choosing $\delta$}
So far we have assumed that the minimum probability $\delta$ is either given or is $O\pn{\frac{1}{n}}$, but a natural choice in applications when estimating $\pi_s[t]$ is to set $\delta = \pi[t]$.  The motivation for this is that if $\pi_s[t] < \pi[t]$, then $s$ is less interested in $t$ than a random source is, so it is not useful to quantify just how (un)interested $s$ is in $t$.  %(More generally we can set $\delta = a \pi[t]$ for some constant $a$.)
%  If we set $\delta = \pi[t]$ we get running time
%\[O \pn{ \frac{1}{\alpha \epsilon}\sqrt{ c m }}. \]

\subsubsection{Generalization}
Bidirectional-PageRank extends naturally to generalized PageRank using a source distribution $\sigma$ rather than a single start node -- we simply sample an independent starting node from $s$ for each walk, and replace $p^t[s]$ with %the expected value of $p^t[s]$ when $s$ is sampled from the starting distribution
$\sum_{v \in V} p^t[v] s[v]$ where $s[v]$ is the weight of $v$ in the start distribution $s$.  It also generalizes naturally to weighted graphs if we simply use the weights when sampling neighbors during the random walks.  For a generalization to other walk distributions or to any given walk length, see Chapter \ref{sec:mc_chapter}.





